Statistical Testing under Distributional Shifts

In this work, we introduce statistical testing under distributional shifts. We are interested in the hypothesis $P^* \in H_0$ for a target distribution $P^*$, but observe data from a different distribution $Q^*$. We assume that $P^*$ is related to $Q^*$ through a known shift $\tau$ and formally introduce hypothesis testing in this setting. We propose a general testing procedure that first resamples from the observed data to construct an auxiliary data set and then applies an existing test in the target domain. We prove that if the size of the resample is at most $o(\sqrt{n})$ and the resampling weights are well-behaved, this procedure inherits the pointwise asymptotic level and power from the target test. If the map $\tau$ is estimated from data, we can maintain the above guarantees under mild conditions if the estimation works sufficiently well. We further extend our results to finite sample level, uniform asymptotic level and a different resampling scheme. Testing under distributional shifts allows us to tackle a diverse set of problems. We argue that it may prove useful in reinforcement learning and covariate shift, we show how it reduces conditional to unconditional independence testing and we provide example applications in causal inference.

==> commands.tex <==
% Capital letters
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}

% Convergence in probability and distribution
\newcommand{\convD}{\stackrel{\mathcal{D}}{\longrightarrow}}
\newcommand{\convP}{\stackrel{\mathcal{P}}{\longrightarrow}}

% Graphs
\newcommand{\PA}{\operatorname{PA}}
\newcommand{\scm}{\mathcal{S}}

% Probability
\newcommand{\E}{\mathbb{E}}
\newcommand{\VAR}{\mathbb{V}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\DO}{\operatorname{do}}

% Misc
\newcommand{\mat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\ind}[1]{\mathbbm{1}_{#1}} % Indicator function
\newcommand{\indep}{\mbox{${}\perp\mkern-11mu\perp{}$}}
\renewcommand{\epsilon}{\varepsilon}
\DeclareMathOperator*{\argmin}{{\arg\min}}
\newcommand{\cP}{\mathcal{P}} % Caligraphic P for class of hypotheses
\newcommand{\cQ}{\mathcal{Q}} % Caligraphic P for class of hypotheses
\newcommand{\cX}{\mathcal{X}} % Caligraphic X
\newcommand{\cZ}{\mathcal{Z}} % Caligraphic Z
\newcommand{\bX}{\mathbf{X}} % Data
\newcommand{\bZ}{\mathbf{Z}} % Target data
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n} % bold calligraphic

\newcommand{\widebar}[1]{\bar{#1}} % Define widebars for putting on top of interventions parents. Currently just bars. 

% Names
\newcommand\james[1]{{\color{red}James: #1}}
\newcommand\note[1]{{\color{red}note: #1}}
\newcommand\niklas[1]{{\color{blue}Niklas: #1}}
\newcommand\rmnik[1]{{\color{gray}Remove(Niklas): #1}}
\newcommand\jonas[1]{{\color{orange}Jonas: #1}}
\newcommand\rmj[1]{{\color{gray}Remove(Jonas): #1}}
\newcommand\Rmjs[1]{{\color{gray}Remove(James): #1}}
\newcommand\nikolaj[1]{{\color[HTML]{538f00}{\tiny NT:}#1}}
\newcommand\Rmn[1]{{\color{gray}{\small RM[NT]: #1}}}
\newcommand\rmn[1]{\Rmn{#1}}
\newcommand\new[1]{{#1}}
\newcommand\old[1]{}

==> environments.tex <==
\newtheorem{theorem}{Theorem}

%% Theorems
\theoremstyle{plain}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
\newtheorem*{remark}{Remark}

%% Cleveref referencing
\crefname{assumption}{}{}

% Don't write Equation (1), but (1) 
\crefname{equation}{}{}

% Referencing list items
% Create new environment for assumption list, and set referencing as assumption instead of "Item"
% See this answer https://tex.stackexchange.com/questions/156049/how-can-i-get-cleveref-enumitem-to-print-not-item-e-but-proposition-1
\newlist{assumpenum}{enumerate}{1} % also creates a counter called 'assumpenumi'
\setlist[assumpenum]{label={(A\arabic*)}}
\crefalias{assumpenumi}{assumption}

\newlist{alt-assumpenum}{enumerate}{1} % also creates a counter called 'assumpenumi'
\setlist[alt-assumpenum]{label={(A\arabic*')}}
\crefalias{alt-assumpenumi}{assumption}


==> figures/icp-table.tex <==
Set & Frequency \\ \hline 
$\emptyset$ &$15.4\% (11.6\%)$\\ 
$\{1,2,3,4\}$ &$0.2\% (0.0\%)$\\ 
$\{2\}$ &$54.2\% (40.6\%)$\\ 
$\{2,3\}$ &$26.2\% (42.0\%)$\\ 
$\{2,3,4\}$ &$0.0\% (1.6\%)$\\ 
$\{2,4\}$ &$0.2\% (0.0\%)$\\ 
$\{3\}$ &$3.8\% (4.2\%)$\\ 


==> figures/model_selection_table.tex <==
resampling & oracle & observed \\ \hline 
$0.874 \pm 0.029$ & 1.0 & 0.0 \\ 

==> packages.tex <==
% AMS packages
\usepackage{amsmath,amsthm,amssymb}
\usepackage{dsfont}

%Clever ref
%https://texblog.org/2013/05/06/cleveref-a-clever-way-to-reference-in-latex/
\usepackage[noabbrev,capitalize]{cleveref}

%Package to get indicator function
\usepackage{bbm}

% .. and to get bold calligraphic fonts
\usepackage{bm}
\usepackage{paralist}
%Enumerated lists with lowercase (i)
\usepackage{enumerate}
\usepackage[inline]{enumitem}
% Use roman numbering in enumerate
\setlist[enumerate,1]{label={\roman*)}}

% Get reverse coloneqq
\usepackage{mathtools}

%Graphics
\usepackage{graphicx}

% Graphs
\usepackage{tikz}
\usetikzlibrary{arrows}% To get more arrow heads
\tikzstyle{graphnodesmall} = [circle,draw=black,minimum size=20pt,text centered,inner sep=0.2mm]
\tikzstyle{observedsmall} = [graphnodesmall,fill=white,text=black]
\tikzstyle{unobservedsmall} = [graphnodesmall,fill=white,text=black,style=dashed]

%% distribution tikz
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{arrows.meta}

\usepackage{ifthen} % Get if-statements in figures

% Enable subfigures
\usepackage{caption}
% \usepackage[font=scriptsize]{caption}
\usepackage{subcaption}

% Algorithms
\usepackage{algorithm, algorithmicx}
\usepackage[noend]{algpseudocode}

% Increase line spacing in algorithms
\usepackage{setspace}
\let\Algorithm\algorithm
\renewcommand\algorithm[1][]{\Algorithm[#1]\setstretch{1.0}}

% Centered \not for non-independence
\usepackage{centernot}

% Nicer tables
\usepackage{booktabs}
% References
% \usepackage[
% backend=biber,
% style=authoryear,
% maxcitenames=2,
% giveninits=true,
% uniquename=false,
% autocite=inline,
% natbib
% ]{biblatex}
% \addbibresource{references.bib}
%% Added firstinits, to only show J. Peters in references. 
%% Added uniquename=false, to not show initial letters in references
%% minbibnames=8,
